Learning to Find Common Objects Across Few Image Collections

Given a collection of bags where each bag is a set of images, our goal is to select one image from each bag such that the selected images are from the same object class. We model the selection as an energy minimization problem with unary and pairwise potential functions. Inspired by recent few-shot learning algorithms, we propose an approach to learn the potential functions directly from the data. Furthermore, we propose a fast greedy inference algorithm for energy minimization. We evaluate our approach on few-shot common object recognition as well as object co-localization tasks. Our experiments show that learning the pairwise and unary terms greatly improves the performance of the model over several well-known methods for these tasks. The proposed greedy optimization algorithm achieves performance comparable to state-of-the-art structured inference algorithms while being ~10 times faster. The code is publicly available on https://github.com/haamoon/finding_common_object.

==> more_shortcuts.tex <==

\usepackage{microtype} % not sure whether we use this or not
\usepackage{graphicx}
\usepackage{rotating}
\usepackage{subfigure}
\usepackage{booktabs} % for professional tables
\usepackage{multirow}
\usepackage{caption}

\graphicspath{ {../figures/} }

\def\d{\text{\normalfont d}}

% whether to inlcude proofs
\newif\ifLONG
%\LONGtrue
\LONGfalse
\ifLONG % just print the proof on spot in the long version
\renewenvironment{proofatend}{\begin{proof}}{\end{proof}}
\fi


% Necessary in order to have theorems, propositions, and lemmas use the same counter
\theoremstyle{plain}
\newtheorem{prop}[theorem]{\bf Proposition}
%\newtheorem{lem}[theorem]{\bf Lemma}

% For restating the theorems in the appendix
%\newtheorem*{theorem*}{\bf Theorem}
%\newtheorem*{prop*}{\bf Proposition}
%\newtheorem*{lem*}{\bf Lemma}



